On Reliability of Patch Correctness Assessment

Current state-of-the-art automatic software repair (ASR) techniques rely heavily on incomplete specifications, e.g., test suites, to generate repairs. This, however, may render ASR tools to generate incorrect repairs that do not generalize. To assess patch correctness, researchers have been following two typical ways separately: (1) Automated annotation, wherein patches are automatically labeled by an independent test suite (ITS) - a patch passing the ITS is regarded as correct or generalizable, and incorrect otherwise, (2) Author annotation, wherein authors of ASR techniques annotate correctness labels of patches generated by their and competing tools by themselves. While automated annotation fails to prove that a patch is actually correct, author annotation is prone to subjectivity. This concern has caused an on-going debate on appropriate ways to assess the effectiveness of numerous ASR techniques proposed recently. To address this concern, we propose to assess reliability of author and automated annotations on patch correctness assessment. We do this by first constructing a gold set of correctness labels for 189 randomly selected patches generated by 8 state-of-the-art ASR techniques through a user study involving 35 professional developers as independent annotators. By measuring inter-rater agreement as a proxy for annotation quality - as commonly done in the literature - we demonstrate that our constructed gold set is on par with other high-quality gold sets. We then compare labels generated by author and automated annotations with this gold set to assess reliability of the patch assessment methodologies. We subsequently report several findings and highlight implications for future studies.

==> RQ1_new.tex <==
\subsection{RQ1: Can professional developers agree on patch correctness?} 
In this research question, we investigate the agreement of professional developers when labeling the data via various scenarios. Our purpose for this research question is to establish the ground truth labels with respect to various scenarios so as to be able to investigate the trade-offs when each scenario is applied to later assess the reliability of author labeling and independent test suite in the subsequent sections.

 \begin{table}
 \caption{Results of developer labeling on various scenarios. Row ``Labels'' indicate the number of patches determined as correct/incorrect.  Remaining rows show the kappa values using various methods. Each column indicates a particular scenario that we consider. \label{tbl:rq1}}

 %\vspace{-10pt}
 \setlength\tabcolsep{1.5pt}
 \begin{center}
 {\small
 \begin{tabular}{l|rrrrr}
 \toprule
          &\textbf{Scenario 1} & 
          \textbf{Scenario 2} &  \textbf{Scenario 3} & \textbf{Scenario 4} & \textbf{Scenario 5} 
          \\
      
 \midrule
  Labels      & 11/82 & 0/35 & 2/13 & 4/1 & 0/0 \\
  Fleiss Kappa        & 1 & 0.561 & 0.472 & 0.455 & 0.442\\
  Kripp Kappa        & 1 & 1 & 0.778 & 0.713 & 0.693\\
  Mkappa & 1 & 0.721 & 0.59 & 0.556 & 0.543 \\
 \bottomrule
 \end{tabular}}
 \end{center}
 \vspace{-5pt}
 \end{table} 
 
Recall that each patch is labeled as incorrect, correct, or unknown by five developers independently. We thus ask the following question: 
\begin{tcolorbox}[width=8.5cm]
How many patches of various degrees of agreement were observed? What are the inter-rater reliability scores of participants?
\end{tcolorbox}
Table~\ref{tbl:rq1} shows details of the results for the above question on several scenarios. We describe these scenarios and the results in prose below. 

\textbf{Scenario 1:} The label ``unknown'' is excluded from the result. 

\textbf{Result}: The number of patches that, when removing the ''unknown'' label, all remaining developers agree on the same label of each patch as correct or incorrect is 93 patches (out of 150 in total). Out of these 93 patches, 11 and 82 patches are agreed to be correct and incorrect, respectively. The kappa values of this scenario are all one, indicating that the labels by developers are reliable. 

\textbf{Scenario 2:} The label ``unknown'' is included in the result. 

\textbf{Result}: The number of patches that all developers agree on the same label of each patch as correct or incorrect is 35. We note, however, that these 35 patches are indeed all agreed to be incorrect. The kappa values of this scenario are 0.561, 1, and 0.721, respectively. This also indicates a considerable inter-rater reliability of the developer labeling.  

\textbf{Scenario 3:} One participant's label disagrees with the label assigned by the majority of others in each patch labeling task. In this case, the final label of each patch is decided by a majority voting method, e.g., a patch is considered incorrect if three developers labeled it as incorrect, and the remaining two developers labeled it either as correct or unknown.

\textbf{Result}:  The numbers of patches identified as incorrect and correct are 13 and 2, respectively. The kappa values of this scenario also show that developer labeling is reliable.

\textbf{Scenario 4:} Two participants' label(s) disagrees with the label assigned by the majority of others in each patch labeling task. Again, the majority voting method is used to identify the final label of each patch. 

\textbf{Result}: The numbers of patches identified as incorrect and correct are one and four, respectively.  Similar to previous scenarios, developer labeling is shown reliable via reasonable kappa values.

\textbf{Scenario 5:} Majority voting cannot determine the final label of a patch. 

\textbf{Result}: We found that there are two special cases in the data belonging to this scenario: (1) two participants label a patch as correct, two other participants label the patch as incorrect, and the remaining participant labels the patch as unknown. (2) two participants label a patch as unknown, two other participants label the patch as incorrect, and the remaining participant labels the patch as correct. Since developers cannot reach a concensus, the final labels of these patches are unknown. 

We next ask several sub-questions to clarify and have further insights into the results that we obtained above. We first ask the following question:
\begin{tcolorbox}[width=8.5cm]
What kind of patches participants tend to \textbf{agree} when labeling?
\end{tcolorbox}

For this question, we consider the scenario 1 as described earlier. Recall that 93 (out of total 150) patches have 100\% agreement among developers labeling the patches. We manually investigate these 93 patches to see what could be the characteristics of the patches that lead to the agreement. We found that the 11 (out of 93) patches, which are agreed as correct, share the same property: they are all syntactically the same as the human patches. Also, changes in these patches are made in the same locations as compared to human ones. For the remaining 82 patches, which are agreed as incorrect, we found that they are all syntactically different from the corresponding human patches. Furthermore, the majority of these machine-generated patches are made in different locations as compared to the human patches. Figure~\ref{fig:rq1ex1} depicts examples of patches that are agreed as correct and incorrect. 

We thus believe that participants tend to agree that a patch is correct/incorrect when the patch and the location where it is applied are the same/different as compared to the corresponding human patch.

We next ask the following question:
\begin{tcolorbox}[width=8.5cm]
What kind of patches participants tend to \textbf{disagree} when labeling?
\end{tcolorbox}

For this research question, we consider scenario 3, 4 and 5 described previously. [Bach:] I see no clear properties that we can derive here. I think the guy(s) who disagrees with other must have made random decision on his own damn luck. Need to check with Lingfeng on who is the guy, is it the same guy that disagrees on many patches.

We next ask the following question:
\begin{tcolorbox}[width=8.5cm]
What kind of patches participants need short/long time to decide whether they are correct or incorrect?
\end{tcolorbox}
We manually analyze the average time needed for labeling each patch based on time recorded per participant. As such, the shortest and longest time for labeling are 7 and 164 seconds, respectively. The average time over all patches is 44 seconds. We observed that machine patches, which are syntactically the same/different and made at the same/different locations as compared to human patches, are often labeled as incorrect very quickly (below 44 seconds). On the other hand, patches that are made at proximate locations to human patches often take longer time for developers to inspect and decide. Consider examples in Figure~\ref{fig:rq1ex1} again, the first patch made by GenProg is syntactically the same as human one. We believe that it is obviously easy for developer to quickly decide (in 12 seconds on average). The second patch made by GenProg is proximate to the location of the human patch, but syntactically different. We believe that the proximity similarity and syntactical differences of the patches have caught developers more attention and required them much more time to examine and decide (in 111 seconds on average).

\lstset{language=Java}
\definecolor{dkgreen}{rgb}{0,0.5,0}
\definecolor{dkred}{rgb}{0.5,0,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\lstset{
basicstyle=\ttfamily\bfseries\scriptsize,
  morekeywords={virtualinvoke}, 
  keywordstyle=\color{blue},
  ndkeywordstyle=\color{red},
  commentstyle=\color{dkred},
  stringstyle=\color{dkgreen},
  numbers=left,
  breaklines=true,
  numberstyle=\ttfamily\footnotesize\color{gray},
  stepnumber=1,
  numbersep=10pt,
  backgroundcolor=\color{white},
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  xleftmargin=.23in
}
%Patch 29 and 1
\begin{figure}
\begin{lstlisting}[frame=none,mathescape=true]
//------ A patch by GenProg that is agreed as correct-----
// Human patch
  if (real == 0.0 && imaginary == 0.0) {
+    return INF;
-    return NaN;
  }
// GenProg patch
  if (real == 0.0 && imaginary == 0.0) {
-    return NaN;
+    return org.apache.commons.math3.complex.Complex.INF;
  }

//------ A patch by GenProg that is agreed as incorrect-----   
// Human patch
 CategoryDataset dataset = this.plot.getDataset(index);
+ if (dataset == null) {
- if (dataset != null) {
     return result;
  }               
// GenProg patch
 CategoryDataset dataset = this.plot.getDataset(index);
- if (dataset != null) {
-    return result;
- }
\end{lstlisting}
\vspace{-0.5cm}
\caption{Examples of patches that participants tend to agree as correct or incorrect.}
\label{fig:rq1ex1}
\vspace{-10pt}
\end{figure}

==> RQ4.tex <==
\begin{comment}
(measured in time) to label as compared to other patches. The p-value for this comparison is 0.0026 ($<$ 0.05), indicating that it is significant. Thus, we can conclude that the null hypothesis $\mathcal{H}_{1}^{null}$ can be rejected in the MAJOR-AGREE ground truth dataset. This implies that potential biases in authors annotation of difficult patches exist.

characteristic
Our results showed that authors annotation is reasonably reliable as compared to the ground truths. However, a natural question arises: is authors annotation consistent with the ground truths only in cases (patches) that are easy to label? The skepticism is that for cases (patches) that are harder to decide the labels, authors may subjectively give different (wrong) labels to the patches as compared to the ground truths, introducing potential biases. We use time taken developers to label patches as a proxy to measure the difficulty of labeling patches (or lack thereof). We thus have the following hypotheses:

(Null hypothesis) $\mathcal{H}_{1}^{null}$:
Authors annotate labels fairly for all patches either whether the patches are hard or easy to decide.

(Alternate hypothesis) $\mathcal{H}_{1}$: Authors annotate wrong labels (as compared to ground truth labels) to patches that are harder to decide (or, in other words, which take longer time to decide).

Figure~\ref{fig:rq2allagree} depicts the box lot showing the comparisons of authors annotation with the ALL-AGREE ground truth. According to the figure, patches that authors annotate the same and different with the ground truth have almost equal difficulty level (measured in time). However, the p-value for this comparison is 0.14 ($>$ 0.05), indicating that it is not significant. Thus, we can only conclude that the null hypothesis $\mathcal{H}_{1}^{null}$ \emph{may} be true in the ALL-AGREE ground truth dataset.

Figure~\ref{fig:rq2majoragree} depicts the box lot showing the comparisons of authors annotation with the MAJOR-AGREE ground truth. According to the figure, patches that authors annotate the same with the ground truth are easier (measured in time) to label as compared to other patches. The p-value for this comparison is 0.0026 ($<$ 0.05), indicating that it is significant. Thus, we can conclude that the null hypothesis $\mathcal{H}_{1}^{null}$ can be rejected in the MAJOR-AGREE ground truth dataset. This implies that potential biases in authors annotation of difficult patches exist.

\begin{tcolorbox}[width=8.5cm]
Authors annotation is reliable for cases that are easy to decide. However, there exists potential biases in authors annotation of patches that are hard to label (take longer time to label).
\end{tcolorbox}

\begin{table}
 \caption{Inter-rater reliability of authors annotation as compared to ALL-AGREE and MAJOR-AGREE ground truths. \label{tbl:rq2a}}

 %\vspace{-10pt}
 \begin{center}
 {\small
 \begin{tabular}{l|rr}
 \toprule
          &\textbf{All Agree} &
          \textbf{Majority Agree}\\

 \midrule
  Cohen's Kappa      & 0.569 & 0.616\\
 \bottomrule
 \end{tabular}}
 \end{center}
 \vspace{-5pt}
 \end{table}
%\dl{Examples are missing here.}
\end{comment}



==> dataset.tex <==


%purpose of our study is to investigate the effectiveness of using author labeling and independent test suite in assessing patch correctness. We thus choose a set of 150 patches generated by various ASR tools, whose labels by authors of the ACS tool (an ASR tool used in our experiment) are publicly available at.


%The majority of the patches are labeled (by the ACS's authors) as \emph{incorrect}, except ACS's patches itself   (78\% of its patches are labeled as correct by its authors). We also note that the original dataset in~\cite{liu2017identifying} contains 210 patches and their respective labels. 

==> rq1.tex <==
\subsection{RQ1}

\vspace{0.2cm}\noindent{\bf Motivation.} We collect five labels from 3rd party developers for each patch in the experiment.
Then, we need to confirm that the patch labels from 3rd party developers are reliable, which means the developers reach considerable agreement on the results of patch labels.
Thus, we can use these labels for majority voting to determine whether the patches generated by automated program repair is correct or not.

\vspace{0.2cm}\noindent{\bf Approach.} Every patch in our data is identified by five developers. We count the number of patches for which five developers cannot reach an agreement, i.e., there are no more than three developers who give the same answer for a patch. If the five developer reach an agreement, we count the number of majority developers, which could be from 3 to 5.
To measure the reliability of agreement on the labels of these 150 patches by 3rd party developers, we use Fleiss kappa~\cite{fleiss1971measuring}, which could work when assessing the agreement between three or more than raters (5 raters in our study).
Table~\ref{tbl:kappa} shows the interpretations for Kappa values.


\begin{table}
\centering
\caption{The interpretations for Kappa values}
\label{tbl:kappa}
\begin{tabular}{|l|l|}
\hline
\textbf{Kappa Value}              & \textbf{Interpretation}                     \\          \hline
$<0$            & poor agreement                                                   \\ \hline
$[0.01, 0.20]$            & slight agreement                                                   \\ \hline
$[0.21, 0.40]$            & fair agreement                                                   \\ \hline
$[0.41, 0.60]$            & moderate agreement                                                   \\ \hline
$[0.61, 0.80]$            & substantial agreement                                                   \\ \hline
$[0.81, 1.00]$            & almost perfect agreement                                                   \\ \hline
\end{tabular}
\end{table}

\vspace{0.2cm}\noindent{\bf Results.}
We find that there are only two patches for which developers cannot reach an agreement. All the other patches could be assigned a label by majority voting. 
Figure~\ref{fig:labelstat} shows the number of patches with different numbers of developers who have a consistent answer. There are 17 and 131 patches that are labeled as correct and incorrect, respectively. 
For most of patches (123/148$\approx$83\%), developers could reach an agreement with a high consistency, i.e., 4 or 5 developers have the same answer.
Meanwhile, the Fleiss kappa is equal to 0.311, which indicates a fair agreement level. 


\begin{figure}
\centering
\includegraphics[width=0.48\textwidth,draft=false]{labelstat}
 \caption{The number of patches with different numbers of developers who have a consistency answer.}
 \label{fig:labelstat}
\end{figure}

\subsection{RQ2}
\vspace{0.2cm}\noindent{\bf Motivation.}
In this research question, we want to investigate the patch labels of majority voting are consistent with the author labels. 

\vspace{0.2cm}\noindent{\bf Approach.}
Given a patch, we compare the label generated by majority voting with the author label. We also investigate the reason why the two labels are inconsistent by inspecting some inconsistent cases. Furthermore, we compute Cohen' kappa~\cite{cohen1960coefficient} between the majority voting labels and the author labels. Cohen's kappa is a statistic which measures inter-rater agreement for categorical items.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{The confusion matrix for the comparison of majority voting labels with the author labels.}
\label{tbl:rq2}
\begin{tabular}{|l|l|c|c|c|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}}                                                                & \multicolumn{3}{c|}{\textbf{Majority Voting}}           \\ \cline{3-5}
\multicolumn{2}{|l|}{}                                                                                 & \textbf{Correct} & \textbf{Incorrect} & \textbf{Unkown} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Author \\ Label\end{tabular}}} & \textbf{Correct}   & 17               & 8                  & 0               \\ \cline{2-5}
                                                                                  & \textbf{Incorrect} & 0                & 114                & 2               \\ \cline{2-5}
                                                                                  & \textbf{Unknown}   & 0                & 9                  & 0               \\ \hline
\end{tabular}
\end{table}

\vspace{0.2cm}\noindent{\bf Results.}
Table~\ref{tbl:rq2} shows the confusion matrix for the comparison of majority voting labels with the author labels. 
We ignore nine patches whose author label is ``Unknown'' because they cannot be compared with the majority voting. 
Thus, the percentage of the patches that have the same label between majority voting and author is equal to 93.9\% (131/141), which indicates a high consistency.  
There are ten patches that have inconsistent labels between majority voting and author. Eight out of 10 patches have ``correct'' author label. We inspect these patches carefully and find there are two reasons that might cause 3rd party developers give a different answer.
One reason is that developer misunderstand the automatically generated patches. For example, one automatically generated patch (its id is 133 in the dataset) add an if condition \textit{if(53 == 0)} before an statement, which must not be done by human in practice. However, the function of these if condition is equal to delete the statement, which is semantically equal to the patch produced by the human developer.
Another reason is that there are considerably differences between the human patch and the automatically generated patch. For example, the human patch and automatically generated patch in Figure~\ref{fig:examplepatch} (the patch id is 45 in the dataset) look semantically different, since the human patch deletes the whole if condition block, whereas the automatically generated patch just deletes one statement in the block.
Furthermore, the Cohen kappa value between the majority voting labels and the author labels is equal to 0.73, which indicates substantial agreement. 

\begin{figure}
\centering
\includegraphics[width=0.48\textwidth,draft=false]{examplepatch}
 \caption{An example patch pairs.}
 \label{fig:examplepatch}
\end{figure}



